EgoExoLearn: A Dataset for Bridging Asynchronous Ego- and Exo-centric View of Procedural Activities in Real World

Being able to map the activities of others into one's own point of view is one fundamental human skill even from a very early age. Taking a step toward understanding this human ability, we introduce EgoExoLearn, a large-scale dataset that emulates the human demonstration following process, in which individuals record egocentric videos as they execute tasks guided by demonstration videos. Focusing on the potential applications in daily assistance and professional support, EgoExoLearn contains egocentric and demonstration video data spanning 120 hours captured in daily life scenarios and specialized laboratories. Along with the videos we record high-quality gaze data and provide detailed multimodal annotations, formulating a playground for modeling the human ability to bridge asynchronous procedural actions from different viewpoints. To this end, we present benchmarks such as cross-view association, cross-view action planning, and cross-view referenced skill assessment, along with detailed analysis. We expect EgoExoLearn can serve as an important resource for bridging the actions across views, thus paving the way for creating AI agents capable of seamlessly learning by observing humans in the real world. Code and data can be found at: https://github.com/OpenGVLab/EgoExoLearn

==> sec/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% In this section, we show the experiments of cross-view association, cross-view action understanding, and cross-view referenced skill assessment benchmarks.

\subsection{Cross-view Association }



\subsection{Cross-view Action Understanding}



\input{tab/cross_view_tas}


\input{tab/cross_view_sta}


\input{tab/cross_view_lta}

% \subsection{Action Recognition} 

% We evaluate multiple vision-only or vision-language models for the recognition task on our EgoLearner dataset. We develop two evaluation settings, fully-supervised and zero-shot. The former provides a new chance to evaluate the representation ability of the vision encoder, similar to the conventional action recognition. The zero-shot setting is developed to serve as a novel zero-shot classification benchmark for vison-language large models (VLLMs).



% \textbf{Supervised Fine-tuning.} 
% We formulate the Fully-supervised setting to a multi-label classification task. In assessing the performance of fully supervised action recognition, we employ the class-wise and sample-wise multi-label mean Average Precision (mAP) evaluation metric due to the presence of multiple labels per clip. This evaluation protocol is reasonable because it matches the long-tail attribute of daily actions. The table~\ref{tab:AR-finetune} shows that \textbf{balabala}.

% \begin{table}[ht]
% \centering
% \scriptsize
%     \caption{We employ the multi-label mean Average Precision (mAP) evaluation metric due to the presence of multiple labels per clip. This approach aligns with the methodology outlined in \cite{mmit}. Specifically, the term ``Marco'' signifies the calculation of mAP on a class-wise basis, while ``Micro'' corresponds to a sample-wise computation.} 
%  \begin{tabular}{llccccc}
%  \toprule
%   \multirow{2}{*}{View} &\multirow{2}{*}{Model}  & \multicolumn{2}{c}{Val} & \multicolumn{2}{c}{Test}  \\
%   \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
%       & & Verb & Noun  & Verb & Noun  \\
%     \midrule
%    \multirow{3}{*}{Ego}  &   $\text{TSN}_{\text{xxx}}$~\cite{tsn} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%       &  Slowfast$_{\text{4,32}}$~\cite{slowfast} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%       &  MViT$_\text{16}$~\cite{mvit} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%       &  VideoMAE$_\text{16}$~\cite{videomae} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%     \midrule
%        \multirow{3}{*}{Exo}  &   $\text{TSN}_{\text{xxx}}$~\cite{tsn} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%       &  Slowfast$_{\text{4,32}}$~\cite{slowfast} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%       &  MViT$_\text{16}$~\cite{mvit} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%     &  VideoMAE$_\text{16}$~\cite{videomae} & 6.7B & \textbf{22.1} & 19.9 & \textbf{21.6} \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:AR-finetune}

% \end{table}

% \textbf{Zero-shot.}
% We evaluate the zero-shot classification performance of verb and noun subsets.
% For the samples with multiple labels, we simply repeat the samples for testing. We use the 16 prompts from the zero-shot classification on Kinetics~\cite{kinetics} for verb subsets. Furthermore, we have searched for a set of prompts, including \textbf{xxx} text templates, to evaluate the noun subsets. It focuses on the model being verb-agnostic in recognizing the categories of objects being interacted with. These prompts are listed in Table~\ref{xxx}.
% We adopt the testing procedure following CLIP~\cite{clip} and test the vision-language models in terms of Top-1, Top-5, and Top-10 accuracy. We adopt the average of them as the final metric. Two types of VLMs, web-scale and ego-scale, are tested respectively. The Table~\ref{tab:AR-ZS} shows \textbf{balabla}.

% \input{tab/action_recognition_zs}





% \begin{table*}[ht]
% \centering
% \scriptsize
%     \caption{Prompts1}
%  \begin{tabular}{lll}
%  \toprule
%   \# &Verb Prompts & Noun Prompts \\
%     \midrule
%    1&  A photo of action \{\}. & A photo of interacting with \{\}.  \\
%    2&  A picture of action \{\}. & A picture of interacting with \{\}. \\
%    3&  Human action of \{\}.  \\
%    4&  \{\}, an action.  \\
%    5&  \{\} this is an action.  \\
%    6&  \{\}, a video of action.  \\
%    7&  Playing action of \{\}.  \\
%    8& \{\} \\
%    9&  Playing a kind of action, \{\}.  \\
%    10&  Doing a kind of action, \{\}.  \\
%    11&  Look, the human is \{\}.  \\
%    12&  Can you recognize the action of \{\}?  \\
%    13&  Video classification of \{\}.  \\
%    14&  A video of \{\}. & A video of interacting with \{\}. \\
%    15 & The man is \{\}. \\
%    16 & The woman is \{\}. \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:AR-ZS-prompts}

% \end{table*}



% \begin{table*}[ht]
% \centering
% \scriptsize
%     \caption{Prompts2}
%  \begin{tabular}{lll}
%  \toprule
%   \# &Verb Prompts & Noun Prompts \\
%     \midrule
%    1&  A photo of action \{\}. & A photo of interacting with \{\}.  \\
%    2&  A video of action \{\}. & A video of interacting with \{\}. \\
%    3&  He or she is \{\}.  & He or she is interacting with \{\}. \\
%    4&  A person is doing \{\}. &  A person is interacting with \{\}.  \\
%    5&  Look, the human is \{\}.  \\
%    6&  Human action of \{\}.  \\
%    7&  Playing action of \{\}.  \\
%    8&  Video classification of \{\}.  \\
%    9&  Doing a kind of action, \{\}.  \\
%    10&  Playing a kind of action, \{\}.  \\
%    11&  Can you recognize the action of \{\}?  \\
%    12&  \{\}, an action.  \\
%    13&  \{\} this is an action.  \\
%    14&  \{\}, a video of action.  \\
%    15&  An action of \{\} is in the video.  \\
%    16&  There is a person doing \{\} in the video.  \\
%    17&  A photo of a person doing \{\}.  \\
%    18&  A photo of a person performing \{\}.  \\
%    19&  A photo of a person practicing \{\}.  \\
%    20&  A video of a person doing \{\}.  \\
%    21&  A example of a person performing \{\}.  \\
%    22&  A example of a person practicing \{\}. \\
%    23&  A demonstration of a person doing \{\}. \\
%    24&  A demonstration of a person performing \{\}. \\
%    25&  A demonstration of a person practicing \{\}. & A demonstration of a person interacting with \{\}. \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:AR-ZS-prompts}

% \end{table*}

\subsection{Cross-view referenced skill assessment}

\input{tab/skill_assessment}




% \section{Ablation studies}




==> tab/cross_view_lta.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{10pt}
  \begin{tabular}[t]{lccccccccc}
    \toprule
     \multirow{2}{*}{Method}&  \multirow{2}{*}{Gaze} & \multicolumn{2}{c}{Val} & \multicolumn{2}{c}{Test} \\
     \cmidrule(r){3-6}\cmidrule(r){7-10}
     && \multicolumn{1}{c}{Ego} &\multicolumn{1}{c}{Exo}  & \multicolumn{1}{c}{Ego} &\multicolumn{1}{c}{Exo} \\
      % \cmidrule(r){3-4}\cmidrule(r){5-6} \cmidrule(r){7-8}\cmidrule(r){9-10}
     % && ED@10 & N & V & N & V & N & V & N \\
    \midrule 
    Exo-only & \XSolidBrush & 16.5 &\textbf{25.4} & 15.3 & \textbf{23.9} \\
    Ego-only & \XSolidBrush & 17.7 & 16.3& 16.6 & 15.5\\
    Ego-only & \Checkmark & \textbf{21.0}& 18.2 & \textbf{20.0} & 17.4\\
    Ego-only & Center & 18.8 & 15.6 & 17.4 & 15.3\\
    \midrule
    \multicolumn{10}{l}{\emph{Unsupervised Domain Adaption}} \\
    Ego2Exo & \XSolidBrush & 17.9 & 16.5 & 17.0 & 15.9\\
    Exo2Ego & \XSolidBrush & 17.1 & \textbf{22.6} & 16.1 & 21.0\\
    Ego2Exo & \Checkmark & \textbf{18.5}	& 16.2 & 17.2 & 15.7\\
    Exo2Ego & \Checkmark & 18.2	& 23.1 & \textbf{17.6} & \textbf{21.2}\\
    \midrule
    \multicolumn{10}{l}{\emph{Knowledge Distillation}} \\
    Ego2Exo & \XSolidBrush & 17.0 & 24.9 & 15.7 & 24.5\\
    Exo2Ego & \XSolidBrush &18.1 & 15.1 & 16.9 & 15.7\\
    Ego2Exo & \Checkmark & 16.9	& 25.4 & 15.2 & 24.9\\
    Exo2Ego & \Checkmark & 21.0	& 17.4 & 20.5 & 17.4\\
    \midrule
    \multicolumn{10}{l}{\emph{Co-training}} \\
    Ego \& Exo & \XSolidBrush & 18.0 & 25.2 & 16.8 & 24.0\\
    Ego \& Exo & \Checkmark &\textbf{21.7}	& \textbf{25.6} & \textbf{21.0} & \textbf{24.4}\\
    \bottomrule
  \end{tabular}
\vspace{0.5pt}
\caption{Results on cross-view long-term action anticipation benchmark. We report the edit distance of the generated sequence of 8 actions, shortly termed ED@8. }
\vspace{-0.4cm}
\label{tab:lta}
\end{table}

==> tab/cross_view_sta.tex <==
% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4.5pt}
%   \begin{tabular}[t]{lccccccccc}
%     \toprule
%      \multirow{3}{*}{Method}&  \multirow{3}{*}{Gaze} & \multicolumn{4}{c}{Val} & \multicolumn{4}{c}{Test} \\
%      \cmidrule(r){3-6}\cmidrule(r){7-10}
%      && \multicolumn{2}{c}{Ego} &\multicolumn{2}{c}{Exo}  & \multicolumn{2}{c}{Ego} &\multicolumn{2}{c}{Exo} \\
%       \cmidrule(r){3-4}\cmidrule(r){5-6} \cmidrule(r){7-8}\cmidrule(r){9-10}
%      && V & N & V & N & V & N & V & N \\
%     \midrule
%     Exo-only & \XSolidBrush & 30.7 & 27.5 & \textbf{40.9} & \textbf{36.9} & 29.9 & 27.3 & \textbf{40.9} & \textbf{35.8} \\
%     Ego-only & \XSolidBrush & 33.4 & 36.8 & 28.7 & 19.9 & 33.4 & 37.0 & 28.9 & 18.4 \\
%     Ego-only & \Checkmark & \textbf{40.9} & \textbf{43.8} & 37.5 & 35.6 & \textbf{40.5} & \textbf{44.7} & 37.6 & 34.9 \\
%     Ego-only & Center & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     \midrule
%     \multicolumn{10}{l}{\emph{Unsupervised Domain Adaption}} \\
%     Ego2Exo & \XSolidBrush & 00.0 & 29.7 & 34.2 & 27.7 & 00.0 & 29.8 & 35.4 & 27.3 \\
%     Exo2Ego & \XSolidBrush & 31.1 & 30.0 & 00.0 & 37.2 & 30.2 & 29.8 & 00.0 & 37.5 \\
%     Ego2Exo & \Checkmark & 00.0 & 00.0 & 37.5 & 00.0 & 00.0 & 00.0 & 38.6 & 00.0 \\
%     Exo2Ego & \Checkmark & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     \midrule
%     \multicolumn{10}{l}{\emph{Knowledge Distillation}} \\
%     Ego2Exo & \XSolidBrush & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     Exo2Ego & \XSolidBrush & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     Ego2Exo & \Checkmark & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     Exo2Ego & \Checkmark& 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
%     \midrule
%     \multicolumn{10}{l}{\emph{Co-training}} \\
%     Ego \& Exo & \XSolidBrush & 33.9 & 37.0 & \textbf{40.3} & \textbf{49.6} & 33.5 & 37.3 & \textbf{39.6} & \textbf{45.0} \\
%     Ego \& Exo & \Checkmark & \textbf{43.2} & \textbf{43.5} & 40.3 & 37.5 & \textbf{43.8} & \textbf{43.4}& 40.9 & 37.7 \\
%     \bottomrule
%   \end{tabular}
% \vspace{0.5pt}
% \caption{Results on cross-view short-term action anticipation benchmark. We report the class-wise Top-5 Recall. }
% \vspace{-0.4cm}
% \label{tab:association}
% \end{table}

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.5pt}
  \begin{tabular}[t]{lccccccccc}
    \toprule
     \multirow{3}{*}{Method}&  \multirow{3}{*}{Gaze} & \multicolumn{4}{c}{Val} & \multicolumn{4}{c}{Test} \\
     \cmidrule(r){3-6}\cmidrule(r){7-10}
     && \multicolumn{2}{c}{Ego} &\multicolumn{2}{c}{Exo}  & \multicolumn{2}{c}{Ego} &\multicolumn{2}{c}{Exo} \\
      \cmidrule(r){3-4}\cmidrule(r){5-6} \cmidrule(r){7-8}\cmidrule(r){9-10}
     && V & N & V & N & V & N & V & N \\
    \midrule
    Exo-only & \XSolidBrush & 30.7 & 23.5 & \textbf{40.9} & \textbf{42.5} & 29.9 & 23.6 & \textbf{40.9} & \textbf{40.5} \\
    Ego-only & \XSolidBrush & 33.4 & 37.6 & 28.7 & 18.0 & 33.4 & 37.8 & 28.9 & 17.6 \\
    Ego-only & \Checkmark & \textbf{40.9} & \textbf{52.3} & 37.5 & 37.6 & \textbf{40.5} & \textbf{52.8} & 37.6 & 37.6 \\
    Ego-only & Center & 33.4 & 38.8 & 33.1 & 33.7 & 33.2 & 38.6 & 34.1 & 32.7 \\
    \midrule
    \multicolumn{10}{l}{\emph{Unsupervised Domain Adaption}} \\
    Ego2Exo & \XSolidBrush & 34.1 & 38.0 & 34.2 & 28.4 & 33.6 & 38.1 & 35.4 & 28.7 \\
    Exo2Ego & \XSolidBrush & 31.6 & 24.2 & 39.9 & \textbf{42.4} & 30.4  & 23.6 & \textbf{39.2} & 39.8 \\
    Ego2Exo & \Checkmark & \textbf{41.0} & \textbf{53.7} & 37.2 & 37.3 & \textbf{40.8} & \textbf{54.2} & 38.7 & 37.1 \\
    Exo2Ego & \Checkmark & 34.1 & 31.5 & \textbf{40.2} & 42.3 & 33.5 & 31.3 & 39.1 & \textbf{40.1} \\
    \midrule
    \multicolumn{10}{l}{\emph{Knowledge Distillation}} \\
    Ego2Exo & \XSolidBrush & 30.7 & 25.1 & 41.5 & 47.6 & 29.6 & 24.9 & 41.6 & 45.2 \\
    Exo2Ego & \XSolidBrush & 34.6 & 38.3 & 30.1 & 18.9 & 34.0 & 38.4 & 28.6 & 18.6 \\
    Ego2Exo & \Checkmark & 30.6 & 25.3 & 41.0 & 47.1 & 29.9 & 25.0 & 41.2 & 45.1 \\
    Exo2Ego & \Checkmark& 41.2 & 55.9 & 37.0 & 39.8 & 41.0 & 56.1 & 37.7 & 39.1 \\
    \midrule
    \multicolumn{10}{l}{\emph{Co-training}} \\
    Ego \& Exo & \XSolidBrush & 33.9 & 37.3 & \textbf{40.3} & 46.7 & 33.5 & 37.4 & \textbf{39.6} & 44.3 \\
    Ego \& Exo & \Checkmark & \textbf{41.6} & \textbf{52.9} & 39.6 & \textbf{47.9} & \textbf{43.8} & \textbf{53.3}& 40.3 & \textbf{44.4} \\
    \bottomrule
  \end{tabular}
\vspace{0.5pt}
\caption{Results on cross-view short-term action anticipation benchmark. We report the class-wise Top-5 Recall. }
\vspace{-0.4cm}
\label{tab:sta}
\end{table}

==> tab/l1_category.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lcccccccc}
\toprule
             & \multicolumn{2}{c}{F1}& \multicolumn{2}{c}{F2} &\multicolumn{2}{c}{F3} & \multicolumn{2}{c}{F4}  \\ 
             \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}
             & ego &exo & ego &exo & ego &exo & ego &exo  \\ 
             \midrule
            verbs (train) & xxx          & xxx        & xxx     \\
            verbs (val) & xxx          & xxx        & xxx     \\
            verbs (test) & xxx          & xxx        & xxx     \\
            \midrule
            nouns (train) & xxx          & xxx        & xxx     \\
            nouns (val) & xxx          & xxx        & xxx     \\
            nouns (test) & xxx          & xxx        & xxx     \\
            \midrule
            clips (train) & xxx          & xxx        & xxx     \\
            clips (val) & xxx          & xxx        & xxx     \\
            clips (test) & xxx          & xxx        & xxx     \\
            \bottomrule
            
\end{tabular}
% \vspace{-0.5pt}
\caption{The number of categories after various processing stages for verb and noun labels.
}
% \vspace{-0.4cm}
\label{tab:l1-cate}
\end{table}

==> tab/l2_category.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lcccccc}
\toprule
             & \multicolumn{3}{c}{egocentric} &\multicolumn{3}{c}{exocentric}    \\ 
             \cmidrule(r){2-4}\cmidrule(r){5-7}
             & train &val & test &train & val &test  \\ 
             \midrule
            videos & xxx          & xxx        & xxx     \\
            \midrule
            segments & xxx          & xxx        & xxx     \\
            steps & xxx          & xxx        & xxx     \\

            \bottomrule
            
\end{tabular}
% \vspace{-0.5pt}
\caption{The number of categories after various processing stages for verb and noun labels.
}
% \vspace{-0.4cm}
\label{tab:l2-cate}
\end{table}

==> tab/retrieval_val.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
  \begin{tabular}[t]{lccccc}
    \toprule
     \multirow{2}{*}{Method}& \multirow{2}{*}{Gaze}&  \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Hard} \\
     \cmidrule(r){3-4}\cmidrule(r){5-6}
     && Ego2Exo & Exo2Ego & Ego2Exo & Exo2Ego \\
    \midrule
    
    \emph{Zero-shot} \\
    Random  &\XSolidBrush & 28.34 & 35.48 &	12.67 & 14.97\\
    EgoVLP~\cite{egovlp} &\XSolidBrush  & 50.23	& 50.92 &	28.80 &	27.18\\
    LaViLa~\cite{lavila}  &\XSolidBrush & 39.17	 & 45.62 &	22.58 &	24.88 \\
    InternVideo~\cite{internvideo} &\XSolidBrush & 51.61 &	46.08 & 26.95 & 21.20 \\
    EgoVLP~\cite{egovlp} &\Checkmark &  48.15 &	51.15 & 28.80 &	29.72\\
    LaViLa~\cite{lavila}  &\Checkmark & 41.93	& 48.15 &	21.88 &	21.42\\
    InternVideo~\cite{internvideo} &\Checkmark & 56.22 & 54.60 & 30.87 & 32.25\\
    \midrule
    \emph{Fine-tuned} \\
    Exo-only &\XSolidBrush  & 64.52&65.66 & 	42.85 & 41.70\\
    Ego-only &\XSolidBrush & 53.00	& 54.14	&	33.64 & 37.09\\
    Ego-only &\Checkmark  & 52.76&57.37			&34.56	& 38.70 \\
    Ego-only& Center& 44.47	&42.39	&		24.65 & 24.19\\
    \midrule
    %EgoExo  &\XSolidBrush & 65.2&65.7& 55.0 & 50.9\\
    EgoExo  &\XSolidBrush & 58.98 & 64.05& 		42.86 & 45.39\\
    EgoExo &\Checkmark & 67.51 & 67.74	&		47.93 & 48.84\\
    \bottomrule
  \end{tabular}
}
\vspace{-0.5pt}
\caption{Association accuracy on the cross-view association validation set. Remove.}
\vspace{-1em}
\label{tab:association_val}
\end{table}
